OSLO: Automatic Cell Counting and Segmentation for Oligodendrocyte Progenitor Cells

Reliable cell counting and segmentation of oligodendrocyte progenitor cells (OPCs) are critical image analysis steps that could potentially unlock mysteries regarding OPC function during pathology. We propose a saliency-based method to detect OPCs and use a marker-controlled watershed algorithm to segment the OPCs. This method first implements frequency-tuned saliency detection on separate channels to obtain regions of cell candidates. Final detection results and internal markers can be computed by combining information from separate saliency maps. An optimal saliency level for OPCs (OSLO) is highlighted in this work. Here, watershed segmentation is performed efficiently with effective internal markers. Experiments show that our method outperforms existing methods in terms of accuracy.

==> ICIP 2018 (arxiv)/Makefile <==
FILENAME = icip_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done


==> Makefile <==
FILENAME = icip_paper
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf

# PAPERSIZE = a4
PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE)
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

pdf: main
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.7 \
		$(PS_FILE) $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

